Across Scales & Across Dimensions: Temporal Super-Resolution using Deep Internal Learning

When a very fast dynamic event is recorded with a low-framerate camera, the resulting video suffers from severe motion blur (due to exposure time) and motion aliasing (due to low sampling rate in time). True Temporal Super-Resolution (TSR) is more than just Temporal-Interpolation (increasing framerate). It can also recover new high temporal frequencies beyond the temporal Nyquist limit of the input video, thus resolving both motion-blur and motion-aliasing effects that temporal frame interpolation (as sophisticated as it maybe) cannot undo. In this paper we propose a "Deep Internal Learning" approach for true TSR. We train a video-specific CNN on examples extracted directly from the low-framerate input video. Our method exploits the strong recurrence of small space-time patches inside a single video sequence, both within and across different spatio-temporal scales of the video. We further observe (for the first time) that small space-time patches recur also across-dimensions of the video sequence - i.e., by swapping the spatial and temporal dimensions. In particular, the higher spatial resolution of video frames provides strong examples as to how to increase the temporal resolution of that video. Such internal video-specific examples give rise to strong self-supervision, requiring no data but the input video itself. This results in Zero-Shot Temporal-SR of complex videos, which removes both motion blur and motion aliasing, outperforming previous supervised methods trained on external video datasets.

==> Related_Work.tex <==
\subsection{Related Work}
Video super resolution is comprised of several more basic tasks such as frame interpolation, motion deblurring and removing aliasing. True Space Time Super Resolution (STSR) aims at solving all of these tasks in a unified solution.

\textbf{Frame Interpolation} aims at upsampling a video to a higher frame rate, while not addressing aliasing or deblurring. Recently frame interpolation has gathered much attention with many works showing great results \cite{DAIN,sepconv,nvidia_slomo,Peleg_2019_CVPR,xue2019video} in sharp videos with no motion blur or aliasing. These frame interpolation methods usually rely on optical flow (OF) estimation which cannot be calculated reliably with blur or aliasing, causing the results of such methods to produce weaker results. 

\textbf{Motion Deblurring.}

Papers to write about:\\
Learning to Extract Flawless Slow Motion from Blurry Videos \cite{flawless}\\
Depth-Aware Video Frame Interpolation (DAIN) \cite{DAIN} \\
ZSSR \cite{zssr}\\
Space-Time Super-Resolution from a Single Video \cite{shahar2011STSR}

==> acknowledgments.tex <==
\subsubsection*{Acknowledgments}
The authors would like to thank Ben Feinstein for his \mbox{invaluable} help with getting the GPUs to run in a smooth and computationally efficient way.
This project has received funding from the European Research Council (ERC) under the European Unions Horizon 2020 research and innovation programme (grant agreement No 788535). 
Additionally, supported by a research grant from the Carolito Stiftung. 
Dr Bagon is a Robin Chemers Neustein Artificial Intelligence Fellow.


==> across-dims-Eyal.tex <==
\section{Patch recurrence across dimensions}

In this work we present a new observation on patch recurrence statistics within a single video. Similar to the observations above about making use of patch similarity in the same scale and across-scales in the video’s 3d volume, in this work we observe statistic recurrence of small-scale-patches across-dimensions, i.e. when the spatial and temporal dimensions are swapped 
(see figures \ref{fig:xy_slices}, \ref{fig:ty_slices}, \ref{fig:tx_slices} and \ref{fig:xy_yt_overlap}). This observation holds true both in-scale and across-scales, and can be used in addition to same-dimension similarity for achieving TSR.

\input{figures/fig_xy_slices.tex}
\input{figures/fig_ty_slices.tex}
\input{figures/fig_tx_slices.tex}
\input{figures/fig_xy_yt_overlap.tex}

It was shown in (??) that small ST patches tend to recur in a video’s 3-d volume, both within the input scale as well as across coarser scales in space and time (see figure \ref{fig:space-time-pyramid}). Here we present a new observation: patches recur also across dimensions, i.e., when the spatial and temporal dimensions are swapped.  In figure 1 we see the video volume in x-y-t axes.  Traditionally, we look at a video frame by frame, i.e. as x-y slices: the t is fixed in each frame, and we look at all x-y pixels. Figure \ref{fig:xy_slices} shows such slices. Swapping the spatial and temporal dimensions, we can observe unconventional slices: the x-t and y-t slices, where each frame has a fixed y or x index, and we observe all x-t or y-t pixels respectively. Examples of such frames appear in figures \ref{fig:tx_slices}, \ref{fig:ty_slices}.
This can be thought of as a different direction to scan the 3-d volume. In order to create a yt frame at $x_{i}$, we can vision a vertical scanner in $x_{i}$ at frame t=0. As the traditional video plays through time, the scanner records that column, resulting in the y-t slice of $x_{i}$. We can also “play” this y-t video through x using all y-t slices, similar to playing all x-y frames through time. An example of such frames and videos appears in the supplementary material. Fast movement, or low temporal resolution, will appear in small patches as compressed, aliased samplings of the xy frames, since the video passes quickly past the “scanner”, while slow sub-pixel movement or high temporal resolution will appear in small patches as stretched samplings of the xy frames, since the video passes slowly past the “scanner”. \textcolor{red}{Do we need/have room for an explaining figure?}
A 2-d illustration can be seen in figure \ref{fig:2dBall_Illustration} - A moving 1D object changes its position in time. The temporal frames are a sampling of that continuous object, with a resulting resolution depending on its speed. For start let’s assume the motion speed is 1 pixel per frame ($\frac{\Delta x}{\Delta t}= 1$ ).  If we look at a fixed location $x_{i}$ through time, the entire object moves past this location, and the entire object will be seen in the $x_{i}$ -slice. However, if we sample slower (which is equivalent to a faster motion), we will see an aliased version of the object. The high-resolution version of the object seen in $t_{i}$  can be used to learn how to undo the motion aliasing in this specific video.
\input{figures/2dBall.tex}
For low TR videos the traditional x-y patches contain high-resolution versions of the x-t and y-t patches, giving rise to a rich bank of examples as to how the temporal resolution should be increased.  We make use of this nontraditional internal recurrence of information, in addition to the traditional recurrence within the same dimension, to perform zero-shot Temporal SR (TSR) from a single video. Using this method, we can remove motion blur and aliasing with a light and simple network. Moreover, for high-temporal-resolution videos with sub-pixel motion between frames, the temporal patches contain information in a higher resolution than the original xy frames, and can be exploited for spatial super resolution. This observation of across-dimension similarity may in fact bind spatial-SR and temporal-SR as the same problem, in which we exploit the higher resolution slices for the increasing the resolution on the lower resolution slices, regardless of their orientation.

Figure \ref{fig:across-dims_111} shows a visual demonstration of the across-dimension similarity of small ST patches in 3-d. Each 5$\times$5$\times$3 patch in the original video searches for its top 10 approximate matches using \textcolor{red}{[Quote PATCHMATCH]} in various scaling and sampling scales, both in the original orientation (yxt) and across dimensions (ytx). As seen in the figure, which depicts a 2d slice of the results, a significant portion of the patches found their best matches across dimensions, and as detailed in this section, patches with large motion - the background trees and grass - display significant similarity across dimensions.
\input{figures/fig_across_dims_111.tex}

\textcolor{red}{The following figures will show that patch recurrence across dimensions applies to videos with complex motions as well as with a simple ones. The following video is of a ball falling into a liquid filled glass. It was taken with a slow-motion camera rotating around the scene (6).  In figures 7 and 8 we can see x-t and y-t slices from that video.
(figure ? - the slices of the rotating video)}

==> del_acknowledgments.tex <==
\subsubsection*{Acknowledgments}
The authors would like to thank Ben Feinstein for his \mbox{invaluable} help with getting the GPUs to run in a smooth and computationally efficient way.
This project has received funding from the European Research Council (ERC) under the European Unions Horizon 2020 research and innovation programme (grant agreement No 788535). 
Additionally, supported by a research grant from the Carolito Stiftung. 
Dr Bagon is a Robin Chemers Neustein Artificial Intelligence Fellow.


==> del_across-dims-Eyal.tex <==
\section{Patch recurrence across dimensions}

In this work we present a new observation on patch recurrence statistics within a single video. Similar to the observations above about making use of patch similarity in the same scale and across-scales in the video’s 3d volume, in this work we observe statistic recurrence of small-scale-patches across-dimensions, i.e. when the spatial and temporal dimensions are swapped 
(see figures \ref{fig:xy_slices}, \ref{fig:ty_slices}, \ref{fig:tx_slices} and \ref{fig:xy_yt_overlap}). This observation holds true both in-scale and across-scales, and can be used in addition to same-dimension similarity for achieving TSR.

\input{figures/fig_xy_slices.tex}
\input{figures/fig_ty_slices.tex}
\input{figures/fig_tx_slices.tex}
\input{figures/fig_xy_yt_overlap.tex}

It was shown in (??) that small ST patches tend to recur in a video’s 3-d volume, both within the input scale as well as across coarser scales in space and time (see figure \ref{fig:space-time-pyramid}). Here we present a new observation: patches recur also across dimensions, i.e., when the spatial and temporal dimensions are swapped.  In figure 1 we see the video volume in x-y-t axes.  Traditionally, we look at a video frame by frame, i.e. as x-y slices: the t is fixed in each frame, and we look at all x-y pixels. Figure \ref{fig:xy_slices} shows such slices. Swapping the spatial and temporal dimensions, we can observe unconventional slices: the x-t and y-t slices, where each frame has a fixed y or x index, and we observe all x-t or y-t pixels respectively. Examples of such frames appear in figures \ref{fig:tx_slices}, \ref{fig:ty_slices}.
This can be thought of as a different direction to scan the 3-d volume. In order to create a yt frame at $x_{i}$, we can vision a vertical scanner in $x_{i}$ at frame t=0. As the traditional video plays through time, the scanner records that column, resulting in the y-t slice of $x_{i}$. We can also “play” this y-t video through x using all y-t slices, similar to playing all x-y frames through time. An example of such frames and videos appears in the supplementary material. Fast movement, or low temporal resolution, will appear in small patches as compressed, aliased samplings of the xy frames, since the video passes quickly past the “scanner”, while slow sub-pixel movement or high temporal resolution will appear in small patches as stretched samplings of the xy frames, since the video passes slowly past the “scanner”. \textcolor{red}{Do we need/have room for an explaining figure?}
A 2-d illustration can be seen in figure \ref{fig:2dBall_Illustration} - A moving 1D object changes its position in time. The temporal frames are a sampling of that continuous object, with a resulting resolution depending on its speed. For start let’s assume the motion speed is 1 pixel per frame ($\frac{\Delta x}{\Delta t}= 1$ ).  If we look at a fixed location $x_{i}$ through time, the entire object moves past this location, and the entire object will be seen in the $x_{i}$ -slice. However, if we sample slower (which is equivalent to a faster motion), we will see an aliased version of the object. The high-resolution version of the object seen in $t_{i}$  can be used to learn how to undo the motion aliasing in this specific video.
\input{figures/2dBall.tex}
For low TR videos the traditional x-y patches contain high-resolution versions of the x-t and y-t patches, giving rise to a rich bank of examples as to how the temporal resolution should be increased.  We make use of this nontraditional internal recurrence of information, in addition to the traditional recurrence within the same dimension, to perform zero-shot Temporal SR (TSR) from a single video. Using this method, we can remove motion blur and aliasing with a light and simple network. Moreover, for high-temporal-resolution videos with sub-pixel motion between frames, the temporal patches contain information in a higher resolution than the original xy frames, and can be exploited for spatial super resolution. This observation of across-dimension similarity may in fact bind spatial-SR and temporal-SR as the same problem, in which we exploit the higher resolution slices for the increasing the resolution on the lower resolution slices, regardless of their orientation.

Figure \ref{fig:across-dims_111} shows a visual demonstration of the across-dimension similarity of small ST patches in 3-d. Each 5$\times$5$\times$3 patch in the original video searches for its top 10 approximate matches using \textcolor{red}{[Quote PATCHMATCH]} in various scaling and sampling scales, both in the original orientation (yxt) and across dimensions (ytx). As seen in the figure, which depicts a 2d slice of the results, a significant portion of the patches found their best matches across dimensions, and as detailed in this section, patches with large motion - the background trees and grass - display significant similarity across dimensions.
\input{figures/fig_across_dims_111.tex}

\textcolor{red}{The following figures will show that patch recurrence across dimensions applies to videos with complex motions as well as with a simple ones. The following video is of a ball falling into a liquid filled glass. It was taken with a slow-motion camera rotating around the scene (6).  In figures 7 and 8 we can see x-t and y-t slices from that video.
(figure ? - the slices of the rotating video)}

==> del_introduction_old.tex <==
\section{Introduction}

\textcolor{red}{I think we should have ``problem formulation" -- explain EXACTLY what is temporal super resolution. Then a subsection ``The challenge" -- why it is so challenging product space of all patches and all motions not to mention blur and aliasing. then ``overview" using internal statistics + across dims = it makes no sense to use external learning at all!}

\subsection*{True Temporal Super-Resolution (TSR)}
A video camera has limited temporal resolution determined  by  the  framerate  and by the exposure-time of each frame.  These limit the maximal speed  of  dynamic  events  that  can  be  observed in a recorded video sequence.
When a very fast dynamic event is recorded with a low-framerate camera,  the  resulting  video  suffers  from  severe motion  blur,  and  motion  aliasing.
Motion blur occurs when a fast-moving object change its position w.r.t the camera while the shutter is open. Motion aliasing occurs when the recorded dynamic scene has events with temporal frequencies beyond the Nyquist limit induced by the temporal sampling rate. An example of motion blur and aliasing can be seen in fig \ref{fig:fan_scene_LTR_interp}.
True Temporal Super-Resolution (TSR) aims not only on to increasing framerate but also to recover new high temporal frequencies beyond the temporal Nyquist limit of the input video, thus resolving motion-aliasing and motion-blur. 
For instance, frame interpolation methods applied to the rotating wheel of fig~\ref{fig:motion-blur} would only add new blurry frames preserving the wrong, counter clockwise, aliased motion. In contrast, TSR aims to recover lost high temporal frequencies and sharpen all the frames, not only the added ones. TSR also resolve ... recovering the true clockwise spin directino of the wheel.

\textcolor{red}{add discussion on the difference between ideal LPF in the spatial domain as opposed to poor rect in temporal domain. why spatial SR only needs to recover lost high frequencies but does not deal with resolving aliasing}

%-	Review what people have done; explain the limitations of the current methods –
Many recent methods \cite{DAIN, nvidia_slomo, sepconv} only increase the framerate by performing temporal-Interpolation. This, however, is not true Temporal Super-Resolution. In particular, they cannot undo motion blur, nor motion aliasing (see Fig.~\ref{fig:fan_scene_LTR_interp}), and are indeed mostly applied to videos captured with very short exposure time with little to no motion blur. 
%
Methods for Video Deblurring [REFS] try to remove motion blur from a video, but do not increase the framerate, hence cannot undo any temporal/motion aliasing. 
%
A new recent method \cite{flawless} attempts to do true TSR, by training on an external dataset with examples of motion blur and motion aliasing. However, their method works well only on videos with the similar spatial and temporal statistics as their training data. However, they perform poorly on other natural videos with complex dynamics, severe motion-blur and severe motion-aliasing (see Fig. XXX). 
%
Such failures are not surprising – generating an inclusive dataset of all possible combinations of spatial appearances, scene dynamics, different motion speeds, different framerates, different blurs and different motion aliasing, etc., is combinatorially infeasible. 

% -	Explain our approach 
In this work we propose to overcome these limitations by replacing the External training with Internal training. Small space-time video patches have been shown to recur across different spatio-temporal scales of a single natural video sequence~\cite{Shahar2011STSR}. This strong internal video-prior was used by them for performing Temporal-SR from a single video (using Nearest-Neighbor patch search within the video). Here we exploit this property for training a Deep fully convolutional Network (CNN) on examples extracted directly from the low-framerate input video. Hence extending the paradigm of Deep Internal Learning \cite{zssr, ingan, singan} from single image to video. 
-	We further observe cross-dimension recurrence ….  (figures ~\ref{fig:All_slices}, ~\ref{fig:glass_slices}, ~\ref{fig:across-dims_111}). Video-specific examples, etc.
-	Our approach is fully unsupervised, requiring no training data other than the low-framerate input video itself. This gives rise to true TSR, with SotA results, outperforming methods trained externally on large video datasets.  

We make the following contributions:

\noindent \textbullet Extending internal learning from single image to video.

\noindent \textbullet across dimensions

\noindent \textbullet simple conv model: no motion/optical flow/other ``expert knowledge" ingrained in the model




==> figures/del_fig-motion-blur.tex <==
A naturalistic open source movie for optical flow evaluation\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/x4_00180.png}
    \caption{\textbf{Motion blur:} By increasing temporal resolution by $\times 4$ blurred frames (top) with exposure time is }
    \label{fig:motion-blur}
\end{figure}

==> figures/fig-motion-blur.tex <==
A naturalistic open source movie for optical flow evaluation\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/x4_00180.png}
    \caption{\textbf{Motion blur:} By increasing temporal resolution by $\times 4$ blurred frames (top) with exposure time is }
    \label{fig:motion-blur}
\end{figure}

==> figures/fig_3D_architecture.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/3D_architecture.png}
    \caption{\textbf{The Architecture of the simple 3D network that performs x2 TSR} }
    \label{fig:3D_architecture}
\end{figure}

==> figures/fig_Manufacturing_training_set.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Manufacturing_training_set.png}
    \caption{\textbf{Manufacturing Training Set Across Dimensions:} Creating Internal Training Set based on Internal Across-Dimension Similarity }
    \label{fig:training-set}
\end{figure}




==> figures/fig_Shai_architecture.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/Shai_architecture.png}
    \caption{\textbf{The algorithm: Coarse to fine scheme and Architecture} }
    \label{fig:shai_architecture}
\end{figure}

==> figures/fig_real_LTR_HTR.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/real_LTR_HTR.png}
    \caption{\textbf{True TSR from Video:} Left+Middle: Failures from inadequate video capturing. Middle+Right: Correcting these failures with True TSR }
    \label{fig:real_LTR_HTR}
\end{figure}

==> figures/fig_results.tex <==
\begin{figure*}
\includegraphics[width=\linewidth]{figures/place-holder.png}
\caption{\textbf{Visually comparing TSR results:} Are you still looking at still figures? What are you waiting for? This is a \textit{video} work -- watch the videos in the attached material! }
\label{fig:visual-results}
\end{figure*}

==> figures/fig_spatial_temporal_scales.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/spatial_temporal_scales.png}
    \caption{\textbf{The space-time pyramid, same dimensions:} zzz }
    \label{fig:space-time-pyramid}
\end{figure}

==> figures/fig_tx_slices.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/tx_slices.png}
    \caption{\textbf{2d t-x slices:} Examples of t-x slices at different y's. }
    \label{fig:tx_slices}
\end{figure}

==> figures/fig_ty_slices.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ty_slices.png}
    \caption{\textbf{2d t-y slices:} Examples of t-y slices at different x's. }
    \label{fig:ty_slices}
\end{figure}

==> figures/fig_xy_slices.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/xy_slices.png}
    \caption{\textbf{2d x-y slices:} Examples of x-y slices at different t's. }
    \label{fig:xy_slices}
\end{figure}

==> figures/fig_xy_yt_overlap.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/xy_yt_overlap.png}
    \caption{\textbf{x-y and y-t slices in 3d space} }
    \label{fig:xy_yt_overlap}
\end{figure}

==> figures/table_benchmark_old.tex <==
\begin{table}
    \centering
    \begin{tabular}{r||c|c|c|c|c|}
        \hline
        & \quad \textcolor{red}{\textbf{Ours}} \quad & Flawless \cite{flawless} & DAIN \cite{DAIN} & Nvidia SloMo \cite{nvidia_slomo} & linear interp. \\
         \hline 
         \hline
        pSNR [dB] &  \textbf{26.73}  &  26.21  & 25.65  & 25.61 & 25.51\\
        SSIM & \textbf{0.907} & 0.905 & 0.893 & 0.892 & 0.893 \\
        LPIPS$^\dagger$ \cite{lpips2018} & \textbf{0.160} & 0.176 & 0.199 & 0.194 & 0.201 \\
         \hline
         \multicolumn{6}{l}{\footnotesize $^\dagger$ Note that LPIPS is a \emph{distance} metric -- lower is better.}
    \end{tabular}
    \captionsetup[table]{skip=10pt}
    \caption{\textbf{Comparing $\times$8 TSR results on our newly curated dataset.} 
     \emph{\small When applied to challenging videos with severe motion blur and motion aliasing, frame interpolation methods (e.g., Nvidia SlowMo and DAIN) score significantly lower. However, even methods that were trained to overcome such challenges, but were trained on external datasets (Flawless), struggle to compete on videos that do not represent the typical motions and dynamic behaviors they were trained on. }}
    \label{tab:benchmark_old}
\end{table}

==> internal_learning.tex <==
\subsection{Internal Learning and Self-Supervision}
\textcolor{red}{Explain briefly the concept of internal learning and self supervision. Bring some noticeble works that show this concept.\\}
Supervised CNNs for super-resolution train on a large external dataset, consisting of low resolution (LR) and high resolution (HR) examples.
These networks are extremely large and complex since they need to learn all possible LR-HR relations, so that they can generalize to new test data. \textcolor{red}{This not only requires extensive training and intricate networks, but also assumes that the images at test time are of similar statistics as the training set.}
Unsupervised methods
\textcolor{blue}{we use "self-supervised" and "unsupervised" interchangeably. Probably better to choose one.}
exploit the internal statistics of a single image
\textcolor{red}{/video}
to perform image super-resolution \cite{zssr, DIP, PPZSSR}.
In \cite{zssr} a simple image-specific CNN is trained to recover the input image from a downscaled version of it. At test time, the network is applied to the input image, to obtain super-resolution.
% , denoising\cite{DIP} and image decomposition \cite{DoubleDIP}.
Similarly, our internal video-specific CNN leverages on the power of cross-scale and cross-dimension internal recurrence of information to recover fine details, undo motion blur and motion aliasing, using a very simple network. The network is trained on temporally
\textcolor{red}{not only temporally. maybe just "downscaled?"}
downscaled versions of the input, and applied to the input video at test time.


\textcolor{red}{ADD A FIG. EXPLAINING SELF-SUPERVISION????}

==> introduction_old.tex <==
\section{Introduction}

\textcolor{red}{I think we should have ``problem formulation" -- explain EXACTLY what is temporal super resolution. Then a subsection ``The challenge" -- why it is so challenging product space of all patches and all motions not to mention blur and aliasing. then ``overview" using internal statistics + across dims = it makes no sense to use external learning at all!}

\subsection*{True Temporal Super-Resolution (TSR)}
A video camera has limited temporal resolution determined  by  the  framerate  and by the exposure-time of each frame.  These limit the maximal speed  of  dynamic  events  that  can  be  observed in a recorded video sequence.
When a very fast dynamic event is recorded with a low-framerate camera,  the  resulting  video  suffers  from  severe motion  blur,  and  motion  aliasing.
Motion blur occurs when a fast-moving object change its position w.r.t the camera while the shutter is open. Motion aliasing occurs when the recorded dynamic scene has events with temporal frequencies beyond the Nyquist limit induced by the temporal sampling rate. An example of motion blur and aliasing can be seen in fig \ref{fig:fan_scene_LTR_interp}.
True Temporal Super-Resolution (TSR) aims not only on to increasing framerate but also to recover new high temporal frequencies beyond the temporal Nyquist limit of the input video, thus resolving motion-aliasing and motion-blur. 
For instance, frame interpolation methods applied to the rotating wheel of fig~\ref{fig:motion-blur} would only add new blurry frames preserving the wrong, counter clockwise, aliased motion. In contrast, TSR aims to recover lost high temporal frequencies and sharpen all the frames, not only the added ones. TSR also resolve ... recovering the true clockwise spin directino of the wheel.

\textcolor{red}{add discussion on the difference between ideal LPF in the spatial domain as opposed to poor rect in temporal domain. why spatial SR only needs to recover lost high frequencies but does not deal with resolving aliasing}

%-	Review what people have done; explain the limitations of the current methods –
Many recent methods \cite{DAIN, nvidia_slomo, sepconv} only increase the framerate by performing temporal-Interpolation. This, however, is not true Temporal Super-Resolution. In particular, they cannot undo motion blur, nor motion aliasing (see Fig.~\ref{fig:fan_scene_LTR_interp}), and are indeed mostly applied to videos captured with very short exposure time with little to no motion blur. 
%
Methods for Video Deblurring [REFS] try to remove motion blur from a video, but do not increase the framerate, hence cannot undo any temporal/motion aliasing. 
%
A new recent method \cite{flawless} attempts to do true TSR, by training on an external dataset with examples of motion blur and motion aliasing. However, their method works well only on videos with the similar spatial and temporal statistics as their training data. However, they perform poorly on other natural videos with complex dynamics, severe motion-blur and severe motion-aliasing (see Fig. XXX). 
%
Such failures are not surprising – generating an inclusive dataset of all possible combinations of spatial appearances, scene dynamics, different motion speeds, different framerates, different blurs and different motion aliasing, etc., is combinatorially infeasible. 

% -	Explain our approach 
In this work we propose to overcome these limitations by replacing the External training with Internal training. Small space-time video patches have been shown to recur across different spatio-temporal scales of a single natural video sequence~\cite{Shahar2011STSR}. This strong internal video-prior was used by them for performing Temporal-SR from a single video (using Nearest-Neighbor patch search within the video). Here we exploit this property for training a Deep fully convolutional Network (CNN) on examples extracted directly from the low-framerate input video. Hence extending the paradigm of Deep Internal Learning \cite{zssr, ingan, singan} from single image to video. 
-	We further observe cross-dimension recurrence ….  (figures ~\ref{fig:All_slices}, ~\ref{fig:glass_slices}, ~\ref{fig:across-dims_111}). Video-specific examples, etc.
-	Our approach is fully unsupervised, requiring no training data other than the low-framerate input video itself. This gives rise to true TSR, with SotA results, outperforming methods trained externally on large video datasets.  

We make the following contributions:

\noindent \textbullet Extending internal learning from single image to video.

\noindent \textbullet across dimensions

\noindent \textbullet simple conv model: no motion/optical flow/other ``expert knowledge" ingrained in the model




==> old_experiments.tex <==
We experimented on challenging videos with severe motion blurs induced by highly non-rigid motions, as well as severe motion aliasing.  We compared our results, both visually and numerically, to the leading methods in the field (DAIN~\cite{DAIN},  NVIDIA SloMo~\cite{nvidia_slomo} and Flawless\cite{flawless}). 
Unfortunately, we could not compare to the TSR work of~\cite{Shahar2011STSR}, due to outdated dysfunctional software . 
%technical issues arising from their outdated software libraries, which made the software dysfunctional. 


Fig.~\ref{fig:visual-results} displays a few such examples for TSR$\times$8. 
% Our results are compared to the leading methods in the field (DAIN~\cite{DAIN},  NVIDIA SloMo~\cite{nvidia_slomo}, Flawless SloMo~\cite{flawless}).  
As can be seen,  complex dynamic scenes of highly non-rigid objects (splashing water, flickerig fire, etc.) pose a challenge to all methods. Moreover, the rotating fan/wheel, which induce severe motion blur and severe motion aliasing, cannot be resolved  by any of these methods. Not only do the frames remain blurry (which can be seen in the figure), they all recover  a false direction of motion (counter-clockwise rotation), and with a wrong rotation speed.
%(cannot be viewed in the figure). 
%\emph{\textcolor{red}{The reader is urged to see the videos in the Supplementary-Material in order to view these strong aliasing effects.}}
\emph{\textbf{The reader is urged to view the videos in our \href{http://www.wisdom.weizmann.ac.il/\~vision/DeepTemporalSR}{project website} in order to see these strong aliasing effects.}}


% Quantitative Results
We further conducted a quantitative comparison of our method to other SotA slow-motion approaches.
True TSR (as opposed to simple frame interpolation) is mostly in-need when temporal information in the video is severely under-sampled, resulting in motion aliasing. Similarly, very fast  stochastic motions occurring within a long exposure time result in unrecognizable objects.  
In order to emphasise this lacuna of frame interpolation and highlight the true challenges of TSR, we curated a small, yet very challenging, dataset.
This dataset consists of  high quality videos of very complex dynamic scenes, taken with high speed consumer cameras. 
These 10 high framerate videos are used as ``ground truth" for comparison. 
They are then severely blurred and sub-sampled with a large temporal $rect$  and coarse temporal sampling, to simulate a variety of LTR videos with severe motion blur and/or motion aliasing (see \href{http://www.wisdom.weizmann.ac.il/\~vision/DeepTemporalSR}{project website}).
%blurry input videos.

We tested different SotA methods (DAIN~\cite{DAIN},  NVIDIA SloMo~\cite{nvidia_slomo} and Flawless~\cite{flawless}) on these complex LTR input videos, and compared their outputs to the sharp high-framerate ``ground truth" videos.
PSNR values of these methods
%, competing on our benchmark can be seen 
can be found in Table~\ref{tab:benchmark}.
Since Flawless is restricted to $\times$10 temporal expansion (as opposed to the $\times$8 of all other methods), 
we ran it in a slightly different setting, so that their results could be compared to the same ground truth.
%hence their reported results are slightly skewed.
%Unfortunately, we could not compare to the very relevant work of~\cite{Shahar2011STSR}, due to technical issues arising from their outdated software libraries, which made the software dysfunctional. 

The results in Table~\ref{tab:benchmark} indicate that TSR methods (Ours and Flawless~\cite{flawless}) are superior to frame-interpolation methods (DAIN~\cite{DAIN},  NVIDIA SloMo~\cite{nvidia_slomo}).
Moreover, on videos of very complex dynamic scenes, our Zero-Shot TSR outperforms the externally trained TSR of Flawless~\cite{flawless}.
% This indicates that for very complex videos, \emph{video-specific training examples} extracted from the LTR input video, are often more powerful and relevant, than external datasets (which do not necessarily resemble the statistics of the input video at hand). 
%
This indicates that for very complex videos, internal examples extracted from the input video, are  more powerful and relevant than external training datasets (which do not necessarily resemble the statistics of the input video). 



%The table further implies that for very complex dynamic scenes, video-specific training examples (Our TSR) leads to superior results over external training examples using a general video dataset (Flawless~\cite{flawless}). 


\input{figures/table_benchmark.tex}

% \textcolor{red}{Explain how we chose our videos, sufficient movement, blur and exposure/framerate}\\
% To simulate real camera sensor blur i.e. lower temporal resolution we average our test video frames with full exposure time and subsample them by a factor of \textcolor{red}{N} which allows us to quantitatively compare our results against a GT.
% Our dataset is a collection of \textcolor{red}{n} video sequences from the Need For Speed (\textit{NfS}) dataset\cite{galoogahi2017needforspeed}, \textcolor{red}{n} videos we shot with a GoPro Hero 5 at 240FPS and \textcolor{red}{n} videos downloaded from Youtube.
% To emphasis the strength of our internal learning solution we focus on difficult cases with strong blur or aliasing and show that with no external data we outperform the state-of-the-art solutions available.\\
% In the following sections we present two comparison schemes. The first, direct comparison with true TSR, and the second is interpolation and deblurring algorithms run one after the other.
% Since our problem is complex and novel we found only one true TSR algorithm \cite{flawless} for direct comparison. For our second comparison method we use a SoTA interpolation method \cite{DAIN} and deblurring *INSERT DEBLUR ALGO* algorithms. Since running two algorithms might accumulate unwanted artifacts we show the comparison we interpolation done first and then deblurring, and deblurring done first then interpolation. To further show stress this we also show that we outperform interpolation on blurry data and deblurring with no subsample.

% \subsection{True TSR}
% \cite{flawless} present a 10x TSR solution whereas our algorithm allows for powers of 2 TSR, thus we show a comparison of our 8x and 16x TSR to their 10x TSR. 

% \textcolor{red}{1. we cannot run oded for comparison because... 2. we run ours+DAIN+NVIDIA on x8, and DAIN on x10 due to inherent technical ...}

% \begin{table}[h!]
% \begin{center}
% \begin{tabular}{||c|c|c|c||} 
% \hline
% Video/Method & Flawless\cite{flawless} & Our 8x & Our 16x \\ [0.5ex] 
% \hline\hline
% biker\_all\_1 & 28.25/0.968 & 6 & 6 \\ 
% \hline
% bee & 36.92/0.996 & 6 & 6 \\ 
% \hline
% soccer\_ball & 34.50/0.989 & 6 & 6 \\ 
% \hline
% kid\_swing & 32.45/0.988 & 6 & 6 \\ 
% \hline
% billiard\_2 & 35.17/0.984 & 6 & 6 \\ 
% \hline
% rubber & 34.80/0.986 & 6 & 6 \\ 
% \hline
% \#7 & 6 & 6 & 6 \\ 
% \hline
% \#8 & 6 & 6 & 6 \\ 
% \hline
% \#9 & 6 & 6 & 6 \\ 
% \hline
% \end{tabular}
% \end{center}
% \caption{Qualitative comparison of true TSR (PSNR/SSIM)}
% \label{table:1}
% \end{table}

% \subsection{Interpolation \& Deblur}
% In this section we show several comparison methods:
% \begin{itemize}
%   \item Interpolation \(\rightarrow\) Deblur
%   \item Deblur \(\rightarrow\) Interpolation
%   \item Interpolation on blurry images
%   \item Deblurring full frame rate (no subsampling)
% \end{itemize}
% As a baseline we also show the result of linear frame interpolation.

% \begin{table}[h!]
% \begin{center}
%  \begin{tabular}{||L|L|L|L|L|L|L||} 
%  \hline
%  Video Method & Linear & Interp\(\rightarrow\)Deblur & Deblur\(\rightarrow\)Interp & Interp Blurry & Deblur HFPS & our \\ [0.5ex] 
%  \hline\hline
%  \#1 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
%  \#2 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
%  \#3 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
%  \#4 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
%  \#5 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
%  \#6 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
%  \#7 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
%  \#8 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
%  \#9 & 6 & 6 & 6 & 6 & 6 & 6 \\ 
%  \hline
% \end{tabular}
% \end{center}
% \caption{Qualitative comparison (PSNR/SSIM)}
% \label{table:2}
% \end{table}


% \begin{table}
% \begin{tabular}{|L|c|L|}\hline
% one & two & three \\\hline
% This is two line thing and centered & only one line&  \multicolumn{1}{m{3cm}|}{This is justified and may go to second line as well, neatly}\\\hline
%   one & two & three \\\hline
%   one & two & three \\\hline
% \end{tabular}
% \end{table}

% \subsection{Ablation Study}
% Do we want to somehow show the importance of across dims in an ``ablation study"?

==> problem-formulation.tex <==
\subsection{Problem Formulation}
A video camera has limited spatial and temporal resolutions. The spatial resolution is determined by the spatial pixel density in each frame and by the camera's Point Spread Function. These  factors limit the minimal size of spatial features that can be visible in an image. The temporal resolution is determined by the frame-rate and by the exposure-time of the camera. These limit the maximal speed of dynamic events that can be observed in a video sequence.

Temporal Super-Resolution (TSR) aims to recover rapid dynamic events that occur faster than the video-frame rate, and are therefore invisible, blurred or seen incorrectly in the video sequence. The amount and nature of these distortions is set by the the video frame rate, the frame exposure time and the speed of motions of objects in the scene.

The video frame rate is the number of frames captured per second. It sets the time gap between two consecutive frames. The camera integrates the light coming from the scene during the exposure time in order to generate each frame. As a result, fast moving objects produce a noted blur along their trajectory, often resulting in distorted or unrecognizable shapes.

The relations between the low-temporal-resolution (LTR) video and its corresponding high-temporal-resolution (HTR) video
\textcolor{red}{video or scene?}
are blur and subsampling in time:
$L = (H * k_{\Delta t}) \downarrow _{t}$
where L is the LTR video, H is the HTR video and $k_{\Delta t}$ is a rectangular (rect) temporal blur kernel with width $\Delta t$, induced by the exposure time.
If the kernel's width is equal to the time between consecutive frames, the exposure time is called
\textbf{full}
$\Delta t = \frac{1}{\mbox{framerate}}$
The case of full exposure time is illustrated in figure \ref{fig:fullexposure}, while sub-exposure time is illustrated in figure \ref{fig:subexposure}.

The width of $k_{\Delta t}$ sets how much we tend to experience motion blur. If objects in the scene move a distance that's translated to more than a pixel size in $\Delta t$ time, the frame will be blurred. In figure \ref{fig:fanblur} we can observe an illustration of motion blur with full-exposure time.
The frame rate sets how much we tend to suffer from aliasing. The frame rate determines the temporal frequency in which the continuous dynamic scene is sampled. \textcolor{red}{Maybe flip: The frame rate determines the temporal frequency in which the continuous dynamic scene is sampled, and as a result - how much we tend to suffer from aliasing.} If the motion is fast in relation to our sample rate we experience aliasing. Demonstrated in figure \ref{fig:fan_scene_LTR_interp} is a video of a fan rotating clockwise (left). However, if sampled too slow it appears to rotate counter clockwise (middle).


